Numerical Simulation of Phase Transition with the Hyperbolic Godunov-Peshkov-Romenski Model

In this paper, a thermodynamically consistent solution of the interfacial Riemann problem for the first-order hyperbolic continuum model of Godunov, Peshkov and Romenski (GPR model) is presented. In the presence of phase transition, interfacial physics are governed by molecular interaction on a microscopic scale, beyond the scope of the macroscopic continuum model in the bulk phases. The developed two-phase Riemann solvers tackle this multi-scale problem, by incorporating a local thermodynamic model to predict the interfacial entropy production. Using phenomenological relations of non-equilibrium thermodynamics, interfacial mass and heat fluxes are derived from the entropy production and provide closure at the phase boundary. We employ the proposed Riemann solvers in an efficient sharp interface level-set Ghost-Fluid framework to provide coupling conditions at phase interfaces under phase transition. As a single-phase benchmark, a Rayleigh-B\'enard convection is studied to compare the hyperbolic thermal relaxation formulation of the GPR model against the hyperbolic-parabolic Euler-Fourier system. The novel interfacial Riemann solvers are validated against molecular dynamics simulations of evaporating shock tubes with the Lennard-Jones shifted and truncated potential. On a macroscopic scale, evaporating shock tubes are computed for the material n-Dodecane and compared against Euler-Fourier results. Finally, the efficiency and robustness of the scheme is demonstrated with shock-droplet interaction simulations that involve both phase transfer and surface tension, while featuring severe interface deformations.

==> Makefile <==
PROJECT='gpr_paper_23'

LATEX='lualatex'
LATEX_CMD='--shell-escape' # Allow for external TIKZ

BIBTEX='biber'
BIBTEX_CMD='--bblsafechars' # Avoid interpretation of special characters (e.g.\ \ss) and leave it to LaTex. Breaks otherwise in some weird cases

all:
	make complete
	#rubber --unsafe --module xelatex -c 'setlist arguments --shell-escape' -f --pdf -s --synctex --warn=all --jobname=$(PROJECT) $(PROJECT).tex

fast:
	${BIBTEX} ${BIBTEX_CMD} $(PROJECT)
	${LATEX}  ${LATEX_CMD}  $(PROJECT).tex


complete:
	${LATEX}  ${LATEX_CMD}  $(PROJECT).tex
	${BIBTEX} ${BIBTEX_CMD} $(PROJECT)
	${LATEX}  ${LATEX_CMD}  $(PROJECT).tex
	${LATEX}  ${LATEX_CMD}  $(PROJECT).tex


clean:
	rm -f *.aux *.auxlock *.bbl *.bcf *.blg *.ist *.lof *.log *.lot *.xml *.slg *.syg *.syi *.tdo *.toc *.out *.alg *.auxlock *.hbg *.hbi *.hlg *.acn *.acr
	#ls *.tex | rev | cut -c 5- | rev | xargs rubber --clean


run:
	nohup okular --unique $(PROJECT).pdf &

